Zero-Shot Action Recognition from Diverse Object-Scene Compositions

This paper investigates the problem of zero-shot action recognition, in the setting where no training videos with seen actions are available. For this challenging scenario, the current leading approach is to transfer knowledge from the image domain by recognizing objects in videos using pre-trained networks, followed by a semantic matching between objects and actions. Where objects provide a local view on the content in videos, in this work we also seek to include a global view of the scene in which actions occur. We find that scenes on their own are also capable of recognizing unseen actions, albeit more marginally than objects, and a direct combination of object-based and scene-based scores degrades the action recognition performance. To get the best out of objects and scenes, we propose to construct them as a Cartesian product of all possible compositions. We outline how to determine the likelihood of object-scene compositions in videos, as well as a semantic matching from object-scene compositions to actions that enforces diversity among the most relevant compositions for each action. While simple, our composition-based approach outperforms object-based approaches and even state-of-the-art zero-shot approaches that rely on large-scale video datasets with hundreds of seen actions for training and knowledge transfer.

==> method.tex <==

\section{Unseen actions from object-scene compositions}
For our problem, we are given a set of unlabelled videos $V$ and a set of action labels $A$. We seek to find a transformation $f(v |O, S) \in A$ that assigns an action label to unseen video $v$ using two sources of prior knowledge, namely objects $O$ and scenes $S$. To that end, we first construct dense compositions of object and scene pairs, which are then employed to perform action inference. Figure~\ref{fig:intro} highlight the main idea, where objects and scenes are paired and used to infer which actions occur in videos through a semantic transfer from object-scene compositions to actions.
%a set of possible unseen action labels $A$, and a set of test videos $V$. We seek to transfer information from two different train sets, from train set $J$ consisting of images labeled with objects $O$ from the ImageNet shuffle~\cite{Mettes2016}, and from train set $K$ made of images labeled with scenes $S$ from the Places365 dataset~\cite{Zhou2018}.

\subsection{Composition construction}
We consider objects and scenes as an interplay and model this by making paired compositions. Let $C = O \times S$ denote the set of compositions, defined as the Cartesian product between all objects and all scenes. Each composition $c = (c_o,c_s) \in C$ consists of one object and one scene for which we define its semantic embedding vector simply as the sum of its components, \ie,
\begin{equation}
\phi(c) = \phi(c_o) + \phi(c_s),
\label{embcompositions}    
\end{equation}
where $\phi(\cdot) \in \mathbb{R}^{300}$ denotes the semantic embedding function, \eg a word2vec representation~\cite{mikolov2013distributed} or sentence transformers~\cite{Wang2020MiniLM:Transformers}. To be able to perform unseen action recognition, we need two functions, namely a likelihood estimation of a composition in a video and a semantic similarity from composition to action. For the likelihood estimation, let $\mathcal{F}_O$ and $\mathcal{F}_S$ denote deep networks pre-trained on objects $O$ and scenes $S$. Then the likelihood for video $v$ is given as:
\begin{equation}
p(c|v) = p(c_o | v ; \mathcal{F}_O) \cdot p(c_s | v ; \mathcal{F}_S).
\end{equation}
The semantic similarity between an object-scene composition $c$ and an action $a$ is given by a direct cosine similarity from their embedding~\cite{mikolov2013distributed}:
\begin{equation}
s(c, a) = \cos(\phi(c), \phi(a)).
\label{eq:casim}
\end{equation}

\subsection{Unseen action inference}
To assign an action label to an unseen video $v$, we follow object-based action literature~\cite{Jain2015,Mettes2017} and first determine the top $k$ most relevant compositions for each action based on Equation~\ref{eq:casim}. Let $C_a^k$ denote the set with the $k$ most semantically similar compositions for action $a$. Then the score for action $a$ in video $v$ is given as:
\begin{equation}
\ell(a,v) = \sum_{c' \in C_a^k} s(c', a) \cdot p(c'|v).
\end{equation}
Finally, the action prediction is given as:
\begin{equation}
f(v) = \argmax_{a \in A} \ell(a,v).
\end{equation}
Similar to object-based approaches, the action inference is a relatively straightforward combination of likelihood estimation and semantic transfer. The key to our approach is that we use both objects and scenes and we consider them as compositions, which provides empirically stronger results than performing likelihood estimation and semantic transfer for objects and scenes separately.
 
%\subsection{Generic matching setting}
%To obtain scores for each action in a video $v \in V$ we follow the approach devised in~\cite{Jain2015}. We first extend this framework by simply generalizing it in such a way that either objects or scenes can be used independently to obtain a score for each action for each video.

%Given a semantic embedding function $\phi (\cdot)$, and a set of possible classes $G$, we can compute their similarity as in~\cite{Mettes2021}:
%\begin{equation}
%\psi (g,a) = \cos (\phi (g), \phi(a)) \text{ such that } g \in G
%\label{genericsim}
%\end{equation}

%We then consider the set $G_a$ of k most relevant classes to an action class $a$.
%Then, following~\cite{Mettes2021} the scoring function for each video can be defined as 
%\begin{equation}
%l_\text{video}(g,a) = \sum_{g \in G_a} \psi(g,a) \cdot Pr(g|v)
%\label{genericscore}
%\end{equation}
%where $Pr(g|v)$ is represented by the likelihood of class $g$ in a video $v$ as determined by a classifier. 

%As previously mentioned, while this framework has been previously applied to objects by considering $G$ to be made of object classes $O$, it can just as easily be directly applied to scenes by considering $G$ to be composed of scene classes $S$. However, scoring videos based on objects and scenes independently does not fully capture yet the interrelation there might be between the two.

%\subsection{Object-scene compositions}
%To consider the interplay between objects and scenes we need to consider all the possible compositions of objects and scene, $O \times S$. For each element in $O \times S$ we can define its semantic embedding as the sum of embedding $\psi(o)$ for object $o$ and the embedding $\psi(s)$ for scene $s$.
%\begin{equation}
%\phi_\text{comp}(o,s) = \phi(o) + \phi(s)
%\label{embcompositions}    
%\end{equation}

%We can then compute the similarity of a composition to an action as \begin{equation}
%\psi_\text{comp}((o,s),a) = \cos (\phi_\text{comp} (o,s), \phi(a)) \text{ such that } (o,s) \in G
%\label{compositionsim}
%\end{equation}

%On the other hand, the probability of each composition in $O \times S$ can be expressed as the product between the probability of the object in the composition and the probability of the scene in the composition:
%\begin{equation}
%Pr_\text{comp}((o,s)|v) = Pr(o|v) \cdot Pr(s|v)
%\label{probcompositions}    
%\end{equation}

%The probability of a composition is dependent on the probabilities of the elements that make up the composition. By considering $G_a$ as the subset of $O \times S$ of the top $k$ relevant object-scene compositions for action $a$, the action score function can simply be adapted to 

%\begin{equation}
%l_\text{video}(v,a) = \sum_{(o,s) \in G_a} \psi_\text{comp}((o,s),a) \cdot Pr_\text{comp}((o,s)|v)
%\label{compositionscore}
%\end{equation}

\subsection{Diverse selection of top compositions}
For unseen action recognition, a standard approach to determine the top compositions $C_a$ for action $a$ is to select the individual compositions with the highest semantic similarity. An issue for compositions specifically is that this leads to low diversity in either the objects or scenes in the top compositions. Most notably, an object or scene that is highly semantically similar to an action will likely be over-represented in the top compositions, which leads to redundancy. We therefore seek to obtain a selection of top compositions that incorporates joint object and scene diversity.

%Differently from the generic setting in which objects or scenes are considered independently, when using object-scene compositions, we should consider a different choice for generating the subset of top $k$ relevant compositions $G_a$. While in the generic setting this is simply the top $k$ objects or scenes based on the cosine similarity, in the compositions setting there might be more redundancy. This is due to the fact that if, for a certain action, either one object or one scene is particularly similar, many compositions containing that one object or scene might be found in the top $k$ compositions.

To obtain diverse top compositions, we take inspiration from information retrieval literature~\cite{chowdhury2010introduction}, specifically Maximum Marginal Relevance~\cite{Carbonell1998TheSummaries}. For action $a$, we start by selecting the most semantically relevant composition, \ie $C_a^\star = \{\argmax_{c \in C} s(c,a) \}$. We then iteratively add the composition that is most semantically similar to action $a$ and least semantically similar to the compositions in $C_a^\star$. Hyperparameter $\lambda$ controls the relative weight of semantic similarity and diversity, where $\lambda=1$ denotes the baseline setting where only semantic similarity to the action is taken into account. The update rule for Maximum Marginal Relevance in this context is given as:
\begin{equation}
C_a^\star := C_a^\star\ \cup\ \argmax_{c' \in C \setminus C_a^\star} \bigg[ \lambda \cdot s(c', a) - (1-\lambda) \cdot \max_{c'' \in C_a^\star} s(c', c'')\bigg].
\end{equation}
We perform the above iterative update rule to populate $C_a^\star$ until it contains $k$ compositions.
%In order to make up for the additional redundancy introduced by considering compositions, we employ the Maximal Marginal Relevance (MMR) ranking method~\cite{Carbonell1998TheSummaries} to diversify the top $k$ compositions. MMR gradually fills up the top $k$ by adding documents one by one. After the first most relevant document is added, MMR iteratively adds onto the ranking list the new document that is most relevant and at the same time least similar to the documents already present in the ranking list. This trade-off between relevance and similarity to the previously added documents is controlled by a parameter $\lambda \in [0,1]$. When $\lambda=1$, the ranking is done solely based on the relevance, while for lower values of $\lambda$ more dissimilar documents are preferred.

%When applied to object-scene compositions in our setting MMR can be expressed as follows:

%\begin{align*}
%MMR =^\text{def} \arg\max_{(o,s)_i \in G_a \backslash G_b} \biggl[ \lambda(\cos(\phi_\text{comp}((o,s)_i), \phi(a) \\
%- (1-\lambda)\max_{(o,s)_j \in G_b} \cos(\phi_\text{comp}((o,s)_i), \phi_\text{comp}((o,s)_j))\biggr]
%\label{MMRforcombs}
%\end{align*}

%~\cb{$G_b$ is already in itself a subset of G, it's the top q (with q being $5*k$) documents that I used since I cannot compute the pairwise cosine similarity for all the documents in G. How should I put this, since this is something that is actually changing in the methods, but simply because of issues with my computing power?}

%~\cb{Also, I use (o,s) all throughout the methods to indicate an element of G to try and convey the fact that it's a composition of two elements now, but I can see how it might not be super clear, especially when I use it in the MMR formula with the i and j subscripts. Do you have any advice about whether I should leave it like that or change it to like a single letter?}
